DXSLAM: A Robust and Efficient Visual SLAM System with Deep Features

A robust and efficient Simultaneous Localization and Mapping (SLAM) system is essential for robot autonomy. For visual SLAM algorithms, though the theoretical framework has been well established for most aspects, feature extraction and association is still empirically designed in most cases, and can be vulnerable in complex environments. This paper shows that feature extraction with deep convolutional neural networks (CNNs) can be seamlessly incorporated into a modern SLAM framework. The proposed SLAM system utilizes a state-of-the-art CNN to detect keypoints in each image frame, and to give not only keypoint descriptors, but also a global descriptor of the whole image. These local and global features are then used by different SLAM modules, resulting in much more robustness against environmental changes and viewpoint changes compared with using hand-crafted features. We also train a visual vocabulary of local features with a Bag of Words (BoW) method. Based on the local features, global features, and the vocabulary, a highly reliable loop closure detection method is built. Experimental results show that all the proposed modules significantly outperforms the baseline, and the full system achieves much lower trajectory errors and much higher correct rates on all evaluated data. Furthermore, by optimizing the CNN with Intel OpenVINO toolkit and utilizing the Fast BoW library, the system benefits greatly from the SIMD (single-instruction-multiple-data) techniques in modern CPUs. The full system can run in real-time without any GPU or other accelerators. The code is public at https://github.com/ivipsourcecode/dxslam.

==> review.tex <==
Reviewer 1 of IROS 2020 submission 1979
======================
% Dongjiang add explanation(done---原文相关位置进行了注释)
1. The reason why the authors adopted HF-Net as feature
extractor is unclear. As shown in Fig.2, D2+BRIEF seems
comparable to HF+HF, even better in some scenes. Why select
HF+HF as the final module of DXSLAM? Is it because of the
easy implementation? or other significant reasons? 
% perf （perf是啥意思，要我干点啥，松哥）
2. Though the rough running time of DXSLAM is mentioned in
the paper, the running time comparison with other SLAM
systems (e.g., ORB-SLAM2, DS-SLAM, D2+BRIEF) is still
necessary. 
% Dongjiang 看看需要吗？我感觉轨迹说明不了问题，后面提到的代表图片更重要(赞同)
4. As a SLAM system, it is expected to see the constructed
maps for each scene while comparing with other SLAM
systems. 
================================
% perf
•	It is mentioned in Section III.B that the
re-implemented feature extraction based on Intel OpenVINO
can achieve over 30 FPS. However, the FPS for the whole
SLAM system is not mentioned, which I think is necessary to
support the real-time performance claim in this paper.
% Dongjiang add explanation（done---原文相关位置进行了注释）
•	In Section IV.B, discussions and explanations of
the feature evaluation results are not enough. Though
figure 2 shows us the experiment results of various feature
extraction approaches on different datasets, it is unclear
to me why the HF feature performs better in some datasets,
while the D2 feature performs better in some other
datasets. I think more explanation about the difference
between those feature extraction methods is needed to let
readers understand well.

================================
% Dongjiang do you have experimental results to support the different
% choice of methods for LCD and re-loc? As the reviewer said,
% "Providing some failing cases on why one
%  approach cannot be used for the other problem may help to
%  better understand the difference"  

%（TODO， I am not sure to give a certain support，but 下面是我的想法）
%这个问题咱们在论文中写了，relocalization不成功的原因，第一种是候选帧不够，第二个主要原因是frame to frame方式匹配的时候，匹配的点数少，就不能relocalization成功，所以采用了global提取更多的frames，同时用frame to map的形式增加匹配点的对数，提高relocalization的成功率.
%至于global的话，global相比于bow具有更多的空间信息，这样检测回环的话相比于完全基于bow更加准确.
%至于下面的审稿人说的100%precision这件事情，relocalization实际中也是不能做到100%precision的吧，我认为LCD要更准，调整累计误差。可以看作本文在relocalization部分放松了些条件，但是我认为，orbslam，使用bow的相似性评分然后去frame 到frame的relocalization也得不到审稿人的100%precision.

Sections III-D, III-E
It is not clear why two different approaches should be used
for localization and loop closure detection. In
localization, global descriptors are compared first, then
local desccriptors are used for pose estimation with images
from the selected group based on global descriptors. In
loop closure detection, BoW approach with local descriptors
is done first, then global descriptors are used to accept
the best hypothesis against the canditates found by BoW.
The only explanation is from this quote of section III-E: 
"Though it [loop closure detection] can also be formed as
an image retrieval problem, its requirement has an emphasis
on precision rather than recall in re-localization, as a
false loop closure may damage the map."
Isn't also the case for localization? We don't want to
localize at the wrong location, so 100% precision would be
also required in localization. About localization, in
section III-D:
"[...] a coarse image retrieval based on the learned global
descriptors, which have been widely verified to be much
more robust to environmental and viewpoint changes than the
BoW method."
Why not using the localization approach in loop closure
detection or vice-versa? It seems to me that in both
approaches a maximum recall at 100% precision would be
required. I assume that if the same approach has not been
used in both localization and loop closure detection, it is
because the author may have done some preliminary
experiments that failed so both approaches needed to be
implemented. Providing some failing cases on why one
approach cannot be used for the other problem may help to
better understand the difference. Both approaches could
have also been compared in the results for the localization
case and then the loop closure detection case.

% Dongjiang 能否挑选几张代表性图片，包括ORB失败但DX成功
%（视角变化和光照不好分别来一组？），和DX也失败的？（done---原文相关位置进行了注释）
Section IV-C:
When it is said: "It fails to re-localize only when where
is a significant viewpoint change [...]" but in conclusion
and introduction it is said that the approach is more
robust to viewpoint. Are there examples where not so
drastic viewpoint changes worked in the presented approach
in constrast to ORB-SLAM2 who would have failed at the same
location(s)? Also, from "It is worth noting that the
robustness against illumination challenges has been greatly
improved.", an example would help the reader to visualize
how much more robust to illimunation the approach is in
comparison to ORB. The video could be referred here.

% Dongjiang 这个我不知道啥意思，酌情吧
Section IV-D:
Can you provide the recall result at 100% precision? This
metric (along with the curves you've shown) is often used
in loop closure detection papers to compare them. The
recall at 100% from FAB-MAP could be added for comparison
with the baseline of the dataset. How the ground truth was
interpreted? Is it that the match is good if it happens
within X images from the real one or within a fixed
distance? Which vocabulary has been used for ORB-BoW, is it
the default one from ORB-SLAM2?

% TODO （这个他好像没有get到点）
Section IV-E
Not sure to understand the difference between the
Per-sequence and Lifelong approaches, because in Figure 5
it says "blue dots indicate successful initialization or
correct re-localization", as in Figure 2 it says "blue dots
indicate successful initialization". So Lifelong is a
combination of re-localizaiton and initialization, why
results in Figure 5 don't have the same performance than in
Figure 2 for initialization part? Would the Figure 5 be
only re-localization? That would make more sense.

% Dongjiang(done---原文相关位置进行了注释)
What is the method used to create the non-incremental
vocabulary for DXSLAM-no-incre?

% Dongjiang(done---原文相关位置进行了注释)
Table II: What really makes DXSLAM more robust to dynamic
environments in comparison to original ORB-SLAM2? Why
dynamic features seem less used in DXSLAM for visual
odometry? Also, having results on same TUM's datasets used
in ORB-SLAM2 paper (like long-office-household, room, 360,
desktop, etc...) could also help to see the differences in
term of accurary between the approaches.

% perf
Section V
As well as claimed in the abstract, introduction and
Section III-A, there are no results to prove that the
approach is actually real-time on CPU. Add subsection in
Section IV to show computation time of the front-end in
comparison to ORB-SLAM2.

======================

% picture
- InTable I, even DXSLAM failed for viewpoint change
(because of 180 degree opposite viewpoint), it is better to
show the images of the big viewpoint change.



